Policy Optimization with Linear Temporal Logic Constraints

We study the problem of policy optimization (PO) with linear temporal logic (LTL) constraints. The language of LTL allows flexible description of tasks that may be unnatural to encode as a scalar cost function. We consider LTL-constrained PO as a systematic framework, decoupling task specification from policy selection, and as an alternative to the standard of cost shaping. With access to a generative model, we develop a model-based approach that enjoys a sample complexity analysis for guaranteeing both task satisfaction and cost optimality (through a reduction to a reachability problem). Empirically, our algorithm can achieve strong performance even in low-sample regimes.

==> old_sec-approach.tex <==
\section{Problem and Approach}

\subsection{Formulation}

% Together with $\mathcal{X}$, a deterministic Markovian policy $\pi(s) = a \in \A(s)$ induces a discrete-time Markov Chain (DTMC). Hence, for a fixed policy $\pi$,  we can partition $\SState = T \cup R_1 \cup \ldots \cup R_k$ where $T$ is a set of transient states and $R_i$ are sets of recurrent states \cite{}. Some $R_i$ must be reached because $T$ is transient, every state $s \in R_i$ will be visited infinitely often and the DTMC will never leave $R_i$. If the set $R_i$ contains states that are accepting in $\mathcal{L}$ then 

Our goal is to find a policy that simultaneously satisfies a given LTL specification with highest probability and is optimal respect to the cost function of the MDP. 
% The desired policy should first satisfy the LTL with highest probability. Then among those policies have lowest cost. 
% We assume we have access to a simulator $\tilde{\X}$ of $\X$ with which we can sample $s' \sim P^{\tilde{X}}(s, a)$ for each state-action pair $(s,a)$. 
% We assume access to a faithful simulator of the true transition function $P$ from which we can sample transitions $s' \sim P(s,a)$ for any state-action pair $(s,a) \in \SState \times \A$.


% , we want to find the one that has smallest average cost (average recurring cost). Then among those policies, we return the one that has smallest transient cost. We include the transient cost because there may be several policies $\pi,\pi'$ that have equal gain and highest probability of LTL satisfaction. Intuitively, $\pi$ may rush to a recurring component and accumulate less cost than $\pi'$, but both still end up in indentical recurring components with equal gain.

Defining the gain (average-cost) and transient cost as
\begin{equation}\label{def:costs}
\begin{split}
g^P_\pi \equiv &\mathbb{E}_{\tau \sim \Tau^P_{\pi}} \left[ \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Cost(s_t, \pi(s_t)) \bigg| \tau \models \varphi \right], \quad J^P_\pi \equiv \mathbb{E}_{\tau \sim \Tau^P_{\pi}}\left[\sum_{t=0}^{\kappa_{\pi}} \Cost(s_t, \pi(s_t)) \bigg| \tau \models \varphi \right],
\end{split}
\end{equation}
% $\Tau^P_{\pi}$ is the set of trajectories induced by $\pi$ in $\X$ with transition function $P$.
where $\kappa_\pi$ is the first, unknown (hitting) time the trajectory $\tau$ leaves the transient states induced by $\pi$. For some $\lambda \geq 0$, the optimal policy is given by 
% \begin{equation}\label{eqn:gain_optimal_policies}
% \begin{split}
% \tilde{\Pi} = \min_{\pi \in \Pi} \; &\mathbb{E}_{\tau \sim \Tau_{\pi}}
% % \left[ \overbrace{\sum_{t=0}^{\kappa_\tau} \Cost(s_t, \pi(s_t))}^{\text{transient}} + \overbrace{\lim_{T \to \infty} \frac{1}{T-\kappa_\tau} \sum_{t=\kappa_\tau}^T \Cost(s_t, \pi(s_t))}^{\text{recurring}} \right] \\
% \left[ \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Cost(s_t, \pi(s_t)) \right] (\equiv \min_{\pi \in \Pi} g_\pi)\\
% &\text{ s.t. } \Prob{\pi \models \varphi} \text{ is maximal} \quad (\text{i.e.} \; \pi \in \arg\max_{\pi \in \Pi} \Prob{\pi \models \varphi})
% \end{split}
% \end{equation}
% where $\Tau_\pi$ is the set of runs induced by $\pi$ in $\X$.
% % and $\kappa_\tau$ is the first time that $\tau$ enters a recurring component $R_i$ induced by $\pi$. 
% We use the shorthand $\mathcal{C}(s, \pi(s)) = \mathbb{E}_{a \sim \pi(s)}[\mathcal{C}(s,a)]$.

% The objective function in \eqref{eqn:main_problem} is commonly known as the average cost or gain. There may be several policies $\pi,\pi' \in \tilde{\Pi}$ that have equal gain and highest probability of LTL satisfaction. Intuitively, $\pi$ may rush to a recurring component and accumulate less cost than $\pi'$, but both still end up in indentical recurring components with equal gain. It may be desirable to pick the one that additionally yields the lower transient cost. Hence, our approach will instead pick:




% % A run $\tau = (s_0, a_0, s_1, a_1, \ldots)$ is a trajectory generated by running $\pi \in \Pi$ in $\mathcal{X}$, where each $s_i = (m_i, q_i)$ is a pair in the product space. Let $\Tau_{\pi}$ be the set of such trajectories. 

% % Since $\Tau_\pi$ forms a probability space, we can quantify the probability that $\pi \in \Pi$ satisfies $\varphi$. Recall, $\varphi$ is satisfied if the automaton states $(q_0, q_1, \ldots)$ within the run $\tau$ are contained in $F \subseteq \SState^\B$ in the LDBA infinitely often. Thus, among all (finitely many) policies $\Pi$ we can first filter on $\tilde{\Pi}$, the ones that satisfy the LTL with highest probability.

% % Next, every $\pi \in \tilde{\Pi}$ induces a Markov Chain together with $\mathcal{X}$ so we can partition $\SState = T \cup R_1 \cup \ldots \cup R_k$ where $T$ is a set of transient states (which are visited finitely often) and $R_i$ are sets of recurrent states (from which runs cannot leave and visit all states infinitely often) \cite{}. Since runs will end up in one of the $R_i$ forever, there will be an average recurring cost of traversing $R_i$. Hence, it is reasonable to look at the average cost of this policy as a criterion for policy discrimination. Ideally, we select a policy within 
% % \begin{equation*}\label{eq:opt_1}
% % \begin{split}
% % \Pi' = \arg\min_{\pi \in \tilde{\Pi}  \subseteq \Pi} \; g_\pi \left( \equiv  \mathbb{E}_{\tau \sim \Tau_{\pi}}\left[\lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^T \Cost(s_t, \pi(s_t)) \right] \right)\\
% % \end{split}
% % \end{equation*}

% % Two policies $\pi, \pi' \in \Pi'$ both have the same probability of LTL satisfaction and average cost, but they differ in their transient cost. Hence, to be slightly more selective, we aim to find
% \begin{equation*}
\begin{align*}
\tag{OPT}\label{eqn:main_problem}
\pi^\ast = \arg\min_{\pi \in \Pi_{\max}} \; &J_\pi + \lambda g_\pi \quad(\equiv V^P_{\pi, \lambda}) &(\text{cost optimal}) \\
\text{ s.t. }\quad &\Pi_{\max} = \left\{\pi\in\Pi \bigg|\ \Prob{\pi \models \varphi} =\max_{\pi' \in \Pi} \Prob{\pi' \models \varphi}\right\} &(\text{prob optimal}) 
\end{align*}
We define $V^P_{\pi, \lambda} \equiv J^P_\pi + \lambda g^P_\pi$. We will often omit the dependence on $P$ and $\lambda$, when unambiguous.  

\begin{prob}[Planning with Generative Model/Simulator]
Suppose access to a generative model of the true dynamics $P$ from which we can sample transitions $s' \sim P(s,a)$ for any state-action pair $(s,a) \in \SState \times \A$. With probability $1-\delta$, for some error $\epsilon >0$, find a policy $\pi \in \Pi$ that simultaneously has the following properties:
\begin{equation}
(i) \;\; \Prob{\pi \models \varphi} = \Prob{\pi^\ast \models \varphi} \quad (ii)\;\; |V_\pi - V_{\pi^\ast}| < \epsilon 
\end{equation}
\end{prob}

% \begin{align*}
% \tag{OPT}\label{eqn:main_problem}
% \pi^\ast = \arg\min_{\pi \in \Pi} \; &V_\pi   &(\text{cost optimal}) \\
% \text{ s.t. }\quad &\pi \in \arg\max_{\pi \in \Pi} \Prob{\pi \models \varphi} &(\text{prob optimal}) 
% \end{align*}
% \end{equation*}


% An astute reader may make the claim that discounting is cleaner and for sufficiently high discount, the discount-optimal policy and the average-cost-optimal policy coincide. While this is true, there is no verifiable way to know if the chosen discount is high enough. As such, we prefer to take an approach with a verifiable formulation. We further believe that our main objective is more easily interpretable than discounted cost.

% We assume we have access to a simulator $\tilde{\X}$ of $\X$ with which we can sample $s' \sim P^{\tilde{X}}(s, a)$ for each state-action pair $(s,a)$. We assume $P^{\tilde{X}} = P^{\X}$, henceforth denoted $P$.





% \hfill
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ Accepting End Components ($\texttt{AEC}$)} 
% 	\label{algo:AEC}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE Simulator $\tilde{\X}$
%     % \STATE Call $\texttt{Sampler}(\phi_{\texttt{AEC}}(\beta), \SState)$
%     \STATE Sample $\phi_{\texttt{AEC}}(\beta)$ times in $\SState \times \A$
%     \STATE $EC = ((A_1, \A_{A_1}), \ldots, (A_m, \A_{A_m})) 
%     % \leftarrow \texttt{AEC}(\X) 
%     \leftarrow \texttt{Algorithm47}((\SState, \A, \widehat{P}))$
%     \STATE Remove $(A_i, \A_{A_i})$ from EC if $A_i \cap \SState^\ast = \varnothing$, not accepting
%     \RETURN $((A_1, \A_{A_1}), \ldots, (A_k, \A_{A_k}))$, AEC
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \hfill
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ $\texttt{Sampler}$ } 
% 	\label{algo:sampler}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE $K \in \mathbb{N}$, a set of states $S$, global $N$ transition tracker
% 	    \FOR{$s \in \SState$}
%             % \STATE $s \leftarrow S.pop()$
%             \FOR{k = 1,\ldots, K}
%                 \STATE Sample $s' \sim P(s,a)$ 
%                 \STATE Track $N(s,a,s') \pp 1, N(s,a) \pp 1$
               
%                 % \STATE If $s'$ is an unseen state, then add $s'$ to $S$ 
%             \ENDFOR
%         \ENDFOR
%     \STATE Set $\hat{P}(s,a,s') = N(s,a,s')/N(s,a)$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}

% \hfill
% \begin{minipage}{.77\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{Value Iteration $(\texttt{VI})$} 
% 	\label{algo:VI}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE Optimistic Bellman Operator $\Bellman$, Error Measure $d$, accuracy $\epsilon > 0$, $S$ states, $S_T$ terminal states, $V_T$ terminal values
% 	    \STATE Set $n=0, v_0 = 0_S, v_1 = \Bellman v_0$
% 	    \REPEAT
% 	        \STATE $n \pp 1$
% 	        \IF{$S_T$ is empty}
% 	            \STATE Shift $v_n \leftarrow v_n - v_n(0)e $ $\COMMENT{\text{Relative Value Iteration}}$
% 	        \ELSE
% 	            \STATE $v_n(s) \leftarrow V_T(s)$ for $s \in S_T$ $\COMMENT{\text{SSP}}$
% 	        \ENDIF
% 	        \STATE Apply operator $v_{n+1}, \tilde{P} \leftarrow \Bellman v_n $ $\COMMENT{\text{Bellman Backup}}$
% 	    \UNTIL{$d(v_{n+1}, v_n) > \epsilon$}
% 	\RETURN $v_{n+1}, v_n, \tilde{P}$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ $\texttt{Filter}$} 
% 	\label{algo:sampler}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE Gains $E=((A_1, g_1),\ldots,(A_k, g_k))$
% 	   %\STATE Set $V_T(s) = 1$ for $s \in \cup_{i=1}^k A_i$
% 	   %\STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, \cup_{i=1}^k A_i, 1)$
% 	   %\STATE Remove $(A_i, g_i)$ from $E$ if $v'(i) \neq \max(v')$
% 	    \STATE $p = 0$, the max probability of reaching
% 	    \STATE Set $G$ as the set of unique $g_i$
% 	    \WHILE{$G$ is not empty}
% 	    \STATE $g \leftarrow min(G)$, $G \leftarrow G\setminus\{g\}$
% 	    \STATE Set $A_g = \cup\{A_k \in E |g_k = g\}$
% 	    \STATE Set $V_T(s) = 1$ for $s \in A_g$
% 	   % \STATE Sample $\texttt{Sampler}(\psi(\rho), \SState \setminus \cup_{i=1}^k A_i)$
% 	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, A_g, V_T)$
% 	   % \STATE Remove $(A_i, g_i)$ from $E$ if $g_i > g$ and $v'(s) = 1$ for $s \in A_i$ arbitrary.
% 	   % \STATE Set $V = v'(s_0)$ for $s \in A_g$ arbitrary
% 	    \IF{$v'(s_0) > p$}
% 	        \STATE Set $p \leftarrow v'(s_0)$
% 	        \STATE Remove $(A_i, g_i)$ from $E$ if $g_i < g$
% 	    \ENDIF
% 	    \ENDWHILE
	    
% 	    \STATE Set $G$ as the set of unique $g_i$
% 	    \WHILE{$G$ is not empty}
% 	    \STATE $g \leftarrow min(G)$, $G \leftarrow G\setminus\{g\}$
% 	    \STATE Set $A_g = \cup\{A_k \in E |g_k = g\}$
% 	    \STATE Set $V_T(s) = 1$ for $s \in A_g$
% 	   % \STATE Sample $\texttt{Sampler}(\psi(\rho), \SState \setminus \cup_{i=1}^k A_i)$
% 	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, A_g, V_T)$
% 	    \STATE Remove $(A_i, g_i)$ from $E$ if $g_i > g$ and $v'(s) = 1$ for $s \in A_i$ arbitrary.
% 	    \STATE Set $V = v'(s)$ for $s \in A_g$ arbitrary
% 	    \IF{$V > p$}
% 	        \STATE Set $p \leftarrow V$
% 	        \STATE Remove $(A_i, g_i)$ from $E$ if $g_i < g$
% 	    \ENDIF
% 	    \ENDWHILE
% 	\RETURN E
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \hfill


\subsection{Intuition, High Level}



We propose a reduction of \eqref{eqn:main_problem} into a reachability problem that can be reduced to an instance of a  Stochastic Shortest Path (SSP) problem and leverage recent literature \cite{Tarbouriech2021, Kolobov2012DeadEnd}. 
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-.6cm}
% \begin{figure}[H]
% \minipage{.5\textwidth}
\begin{center}
  \includegraphics[width=.8\linewidth]{./figs/intuition.pdf}
  \end{center}


\caption{The goal of LTL Constrained Policy Optimization can be reduced to a reachability problem. We want to reach $A_1$ or $A_2$ from $s_0$ and then follow the blue arrows with some distribution. $A_3$ with the blue arrows is a rejecting end component because it does not contain an accepting state $s^\ast$. For $\beta < 1$ , the yellow action is not in the allowable action set of $A_1$ because there is a risk of entering $A_3$, strictly decreasing our probability of LTL satisfaction.}
 \label{fig:intuition}
 \vspace{-.6cm}
% \endminipage
% \end{figure}
\end{wrapfigure}

Consider the accepting states $s_1^\ast, s_2^\ast$ in Figure \ref{fig:intuition}. 
Call the blue arrows the action sets $\A_{A_1}$ and $\A_{A_2}$ in $A_1$ and $A_2$ respectively. The uniform policy over $\A_{A_1}$ and $\A_{A_2}$ will visit the $s_1^\ast, s_2^\ast$ infinitely often, and is probability optimal. % The uniform policy over blue arrows within the enclosing sets $A_1, A_2$ will visit the respective $s^\ast$ infinitely often. Call the blue arrows the action sets $\A_{A_1}$ and $\A_{A_2}$ in $A_1$ and $A_2$ respectively. Fixing this uniform policy over $\A_{A_1}, \A_{A_2}$ is probability optimal within $A_1$ and $A_2$. 
Remaining is the reachability problem of finding a policy that induces low-cost, high probability paths from $s_0$ to $A_1, A_2$. Following the policy returned by SSP, we switch to the uniform policy we developed over $\A_{A_1}, \A_{A_2}$ once we reach $A_1$ or $A_2$ respectively. 

We must be cautious about not selecting the yellow action from $s_1^\ast$ as this enables a chance of reaching set $A_3$, where we get stuck. Hence, the yellow action should not exist in the available actions $\A_{A_1}$. We refer to $(A_1, \A_{A_1})$ as a maximally accepting EC (recall Def \ref{def:end_component}). Similarly, $(A_2, \A_{A_2})$ is also an AMEC. While $(A_3, \A_{A_3})$ is a MEC, it is rejecting. 

Sampling blue arrows uniformly is probability optimal, but may not be cost optimal. Similarly, the cost optimal policy may not be probability optimal. Consider just $A_1$ for the moment. Suppose the cost of the arrows between the white nodes is $4$ while the other costs are $7$. Then the uniform policy in $A_1$ over $\A_{A_1}$ has cost $\frac{1}{2}\left(\frac{4 + 4}{2}\right) + \frac{1}{2}\left(\frac{7 + 7 + 4}{3}\right) = 5$, but is probability optimal. The gain optimal policy that deterministically selects the actions between the white nodes $\tilde{\pi}$ has cost $\left(\frac{4 + 4}{2}\right) = 4$, but is not probability optimal. If we perturb $\tilde{\pi}$ to make it even slightly stochastic (but mostly deterministic, i.e $\eta$-greedy with $\eta \approx 1$) then it will be arbitrarily close to gain optimality and also recover probability optimality. This is a preferable policy over the uniform policy.

At a high level, the procedure is then to (i) identify the AMECs (e.g. $(A_1, \A_{A_1}), (A_2, \A_2))$ by filtering out bad actions like the yellow arrow (ii) find a good policy in each AMEC that visits some $s^\ast$ infinitely often and, finally, (iii) instantiate an SSP problem that finds a policy from $s_0$ to the states $A_1 \cup A_2$ and avoids $A_3$. Stitching together the policies from $(ii)$ and $(iii)$ gives us the cost-efficient policy $s_0$ that visits $s^\ast$ infinitely often, satisfying the LTL specifcation with minimal cost.

% Suppose $A_1, A_2, A_3$ from Figure \ref{fig:intuition} were just states instead of sets of states. Suppose $A_1, A_2$ are the accepting states and $A_3$ is the rejecting state. Then the goal would be to find a policy that induces cost-efficient paths from $s_0$ to $A_1, A_2$ and avoids traps like $A_3$. The case when $A_1, A_2, A_3$ are simply states is a special subset of LTL specifications, when the specification is verifiable in finite sequences.

% We can apply the same principles to full LTL over infinite sequences. In general, $A_1, A_2$ and $A_3$ are sets but we will fix policies in them such that they act as states. Consider $A_1$ for the moment and $\beta < 1$. If the allowable actions in $A_1$, denoted $\A_{A_1}$, does not contain the yellow-dotted action coming from $s_1^\ast$ then $A_1$ is an inescapable set. In particular, uniformly sampling the remaining actions available in $A_1$ leads to visiting $s_1^\ast$ infinitely often. Under this uniform policy, any trajectory reaching $A_1$ satisfies the LTL specification. Hence, fixing a policy in $A_1$ with specific allowable actions $\A_{A_1}$ makes $A_1$ act effectively as a state. This idea can be applied to each $A_i$, reducing us back to the same reachability problem as in the finite case: reach $A_1,A_2$ with maximum probability and follow the random policies thereafter.



% Consider the Figure \ref{fig:intuition}

% Suppose, for a moment, that we only cared about LTL specifications that are verifiable within some finite runs of length $H$: if the logic is satisfied within $H$ time steps then we claim success. We can think of the LTL automaton $\mathcal{B}$ as keeping track of the extent of the specification satisfaction. If we reach an accepting state in the automaton, then we have completed all the requirements of the specification. Similarly, focusing on the product-MDP, if we reach the accepting state then we have completed the specification. Hence, the optimal policy would be one that finds a cost-efficient path to these accepting states. Additionally, we want to minimize the probability of falling into any ``traps'' (if they exist), from which there was no chance of reaching an accepting state.

% The Stochastic Shortest Path (SSP) problem \cite{Bertsekas} is precisely designed to find cost-efficient paths to specific, pre-designated states. The reduction to an SSP instance involves fixing stochastic policies in the end components and finding a policy that induces cost-efficient paths to those end components.
% A few works \cite{Kobolov} also give preliminary results to find policies in the case of traps, which we build upon.

% We now consider the extension from finite runs to infinite runs, enabling full LTL specifications. Instead of finding a cost-efficient path to specific states, we find a cost-efficient path to specific regions (sets of states). By randomly sampling (specific) actions in these regions, the region is never left and all states will be visited. If the region contains an accepting state, then all runs that enter this region are accepting. We can think of these regions as just a ``large'' accepting state. Now we have a reduction back to an SSP.

% For concreteness, we first sample enough from each state-action pair to be able to calculate the MDP's accepting end components $((A_1,\A_{A_1}),\ldots,(A_k,\A_{A_k}))$. Recall, an end component is a set of recurrent states we can force the system to stay in under a restricted action set. Each end component is a special region for which we will find a partial policy. Uniformly sampling from $\A_{A_i}$ in $A_i$ is sufficient if the desire is only maximum probability of satisfaction. However, there may exist policies with lower gain.
% We compute a gain optimal (partial) policy $\pi_i$ in $A_i$ for each $A_i$. Since $A_i$ is accepting then $\pi_i$ satisfies $\varphi$ with probability $1$ for any starting state $s \in A_i$. 

% If there does not exist a probability $1$ path from $A_i$ to some other $A_j$ where the gain of $\pi_j$ is smaller than the gain of $\pi_i$ then $\pi_i$ is gain-optimal, $\pi_i \in \tilde{\Pi}$, and $\pi_i$ agrees with $\pi^\ast$ in $A_i$ (with respect to \eqref{eqn:main_problem}). Hence, in line 5 we filter all of the AEC that are reachable (with probability $1$) from low-gain AECs. 

% The full policy $\pi$ would be to follow transient partial policy $\pi_0$ during the transient part of the states and then, once reaching an end component $A_i$, follow the respective partial policy $\pi_i$. 
% The gain $g_i$ of the end component $A_i$ is thus the terminal cost associated to $\pi$.

% The gain of the end components is the terminal cost associated to any policy in the transient states because the full policy is 

% Now, it suffices to find the policy that balances the cost of the path to the end components with the gain of the end components. In other words, the gain of the end components serves as a terminal cost, as it's the cost of 

% consider the path that balances 

% a greedy policy that induces a lowest-cost path (with highest probability) to the remaining AECs will be a solution to \ref{eqn:main_problem}. We find this policy in line 6.

% All that remains is to find the highest probability, lowest-cost path to the remaining AECs, which we do in line 6.


% It remains to show that $\pi_i \in \tilde{\Pi}$ to verify that indeed $\pi_i$ and $\pi^\ast$ agree on $A_i$.

% For any state $s \in A_i$ there are three outcomes: (i) 


% Suppose a trajectory $\tau$ of $\pi^\ast$ enters $A_i$. Then there are only two choices: (i) $\pi^\ast$ must agree with $\pi$ in terms of gain $A_i$, and $\tau$ will remain in $A_i$ or (ii) there exists a probability $1$ path to some other $A_j$ and $\pi_j$ has lower gain than $\pi_i$. 



% Suppose some trajectory $\tau$ from $\pi$ enters AEC $A_i$. Then, if we desire $\pi \in \tilde{\Pi}$

% $\Prob{\pi \models \varphi} = 1$ and we need 




% Specifically, we want to pick policies that ``quickly'' drive the system to a recurrent set that contains accepting states. Further we want the average cost of traversing the recurrent states to be low. That way, the LTL is satisfied and both the transient cost and recurrent cost is low. 

% One of the main challenges in LTL constrained policy optimization is the verification of constraint satisfaction. Indeed, without knowing any structure of the graph, there is no hope for verification. Recall, the constraint satisfaction is not only reaching an accepting state, but reaching an accepting state infinitely often. To guarantee a state is visited infinitely often, we need to verify that the state is within a recurrent set of states induced by a policy. Inherently, this is dependent on the structure of the MDP.

% Our procedure follows Algorithm \ref{algo:main}. In line 1 we collect enough samples to be able to resolve the constraint satisfaction verification issue. In line 2, we calculate the end components (Line 2) in $\X$ (see def \ref{def:end_component}). These are the sets of states that we can force a system to stay in forever through a restricted set of actions. Among these, we select only those that contain an accepting state, thereby making a run entering this component accepting.


% We find  In Line 4, for a restricted set of states $A_i$, we find a stochastic average-optimal $\pi_i$ that satisfies the LTL with probability $1$. 


% First we achieve enough samples (Line 1) to calculate the end components (Line 2) in $\X$ (see def \ref{def:end_component}). These are the sets of states that we can force a system to stay in forever through a restricted set of actions. Among these, we select only those that contain an accepting state, thereby making a run entering this component accepting. $\pi^\ast$ must agree with the average-optimal policy  

% Then, for each component, we find the optimal average-cost policy 

\subsection{Assumptions, High Prob. Event, and Notation}



% We focus on the specific instantiation of Algorithm \ref{algo:main}. We defer analysis of the algorithm to Section \ref{sec:analysis}. Fix some $\epsilon, \delta > 0$ for which we seek an $\epsilon$ approximation to $\pi^\ast$ with probability $1-\delta$.

% \textbf{Assumptions.} 
% The standard online approach is to start at an initial state $s \sim d_0$, run some policy $\pi$, collect data, and do policy improvement. Unfortunately, due to the nature of the acceptance condition of LTL, 
We discuss the set of assumptions we make prior to diving into the roots of the algorithm. Surprisingly, when planning with a simulator, even infinite data is insufficient to verify an LTL formula without having a known lower-bound on the lowest nonzero probability of the transition function $P$ \cite{Littman2017}. In fact, without this assumption, LTL constrained policy learning is not learnable \cite{Yang2021Intractable}.  

% Furthermore, even with Assumption \ref{assump:lower_bound}, an online approach may take exponential time to verify the satisfaction of the LTL constraints. In order to avoid this, we make the mild assumption that we have access to a simulator, Assumption \ref{assump:simulator}.

\begin{assumption}[Lower Bound]\label{assump:lower_bound}
We assume we have access to a lower bound $\beta > 0$ on the lowest non-zero probability of the transition function $P$:
\begin{equation}
    0 < \beta \leq \min_{s,a,s' \in \SState\times\A\times\SState} \{P(s,a,s') | P(s,a,s') > 0\}
\end{equation}
\end{assumption}

\begin{assumption}[Bounds on cost function]\label{assump:cost_function}
The minimum cost $c_{\min} > 0$ is strictly positive.
\end{assumption}
For simplicity, we need all the costs to be strictly positive. In the presence of negative or zero costs, the SSP reduction may fail to reach the accepting end components due to zero-cost (or negative-cost) cycles. There exist extensions \cite{Tarbouriech2021} to SSP that allow SSP planning in the presence of such cycles through small cost-perturbations. 

% \begin{assumption}[Simulator]\label{assump:simulator}
% We assume that we have access to a simulator that allows us to sample from the transition function $P$. 
% \end{assumption}

% \begin{lem}(High Probability Event)\label{lem:event}
% The following event $\mathcal{E}$ holds with probability at least $1-2\delta$:
% \begin{align*}
% \mathcal{E} &= \{\forall s,a, s' \in S \times A \times S, \forall n(s,a) \geq 1 : | (P^\ast - \widehat{P})(s'|s,a) | \leq \sqrt{\frac{2 \hat{p}(1-\hat{p}) \log(\frac{4 n^2 S^2 A}{\delta})}{n-1}} + \frac{7\log(\frac{4 n^2 S^2 A}{\delta})}{3(n-1)} \} \\
% \end{align*}
% \end{lem}


% Let $\widehat{P}$ be the estimate of 

% We will be keeping track of $\widehat{P}(s,a,s')$, the empirical frequency $N(s,a,s')/N(s,a)$ (line 5 of $\texttt{Sampler}$), the number of times $(s,a)$ transitioned to $s'$. We further assume that the event $\mathcal{E}$ occurs.
We will be keeping track of $\widehat{P}(s,a,s')$, the empirical frequency of visiting $s'$ from state-action pair $(s,a)$. We need to quantify our uncertainty about $\widehat{P}(s,a,s')$. So we introduce the event $\mathcal{E}$, based on empirical Bernstein bounds \cite{Maurer2009}, which holds with probability $1-\delta$ (See Lem \ref{lem:event}).

\begin{restatable}[High Probability Event]{defn}{highProbEvent}
% \begin{defn}[High Probability Event]
\label{def:high_prob_event}
Let $\psi_{sas'}(n) \equiv \sqrt{\frac{2 \hat{P}(s,a,s')(1-\hat{P}(s,a,s')) \log(\frac{4 n^2 |S|^2 |A|}{\delta})}{n-1}} + \frac{7\log(\frac{4 n^2 |S|^2 |A|}{\delta})}{3(n-1)}$ and $\psi(n) \equiv \sqrt{\frac{ \log(\frac{4 n^2 |S|^2 |A|}{\delta})}{2(n-1)}} + \frac{7\log(\frac{4 n^2 |S|^2 |A|}{\delta})}{3(n-1)}$ then define the event 
\begin{equation*}
    \mathcal{E} = \{\forall s,a, s' \in S \times A \times S, \forall n(s,a) \geq 1 : | (P - \widehat{P})(s,a,s') | \leq  \psi_{sas'}(n) \}
\end{equation*}
\end{restatable}

\begin{rem}
$\psi_{sas'}(n)$ is maximized when $\widehat{P}(s,a,s') = \frac{1}{2}$, thus $\psi_{sas'}(n) \leq \psi(n)$ for any $s,s' \in \SState, a \in \A(s)$ and all $n \geq 1$. 
\end{rem}

Under event $\mathcal{E}$ and Assumption \ref{assump:lower_bound} we can form the set of plausible transition functions:

\begin{equation}
    \mathcal{P} = \{ \tilde{P}: \SState \times \A \to \Delta(\SState) | \begin{cases}
    \tilde{P}(s,a,s') = \widehat{P}(s,a,s'), \quad &\widehat{P}(s,a,s') \in \{0,1\}\\
    \tilde{P}(s,a,s') \in \widehat{P}(s,a,s') \pm \psi_{sas'} \cap [\beta, 1-\beta], \quad &\text{otherwise}
    \end{cases}\}
\end{equation} 
Let $\mathcal{P}(s,a) \equiv \{P(s,a,\cdot) | P \in \mathcal{P}\}$ be the possible transition distributions for state-action pair $(s,a)$. 



\subsection{Main Algorithm}

\begin{minipage}{1\textwidth}
\begin{algorithm}[H]
	\begin{small}
	%\renewcommand{\thealgorithm}{}
	\caption{ LTL Constrained Planning (LCP)} 
	\label{algo:main}
	\begin{algorithmic}[1]
	   % \STATE $G \leftarrow \texttt{GetGraph}(\mathcal{X})$
	   %\STATE Set $N = ()$, a global count of the transitions
	    \STATE Sample $ \phi_{\texttt{AEC}}(\beta)$ times in $\SState \times \A$  
	   % and add to $D \leftarrow \{(s,a,s')\}$ $\COMMENT{\text{Get Support of } P}$
	    \STATE Track $\widehat{P}(s,a,s') = \frac{|\{(s,a,s') \in D\}|}{|\{(s,a) \in D\}|}$ \hfill$\COMMENT{\text{Empirical estimate of } P}$
	    \STATE $((A_1, \A_{A_1}), \ldots, (A_m, \A_{A_m})) \leftarrow \texttt{AEC}((\SState, \A, \widehat{P}))$
	    \FOR{$i = 1, \ldots, m$}
	       % \FOR{$s^\ast \in A_i \cap A^\ast$}
	           % \STATE $\pi_{i, s^\ast} , v_{i, s^\ast} \leftarrow PlanRecurrent(A_i, \A_{A_i}, s^\ast)$
	       % \ENDFOR
	       % \STATE $s \leftarrow \arg\min_{s^\ast \in A_i \cap A^\ast} v_{i, s^\ast}$
	       % \STATE Set $\pi_i \leftarrow \pi_{i, s}$
	       \STATE Set $\pi_i, g_i \leftarrow \texttt{PlanRecurrent}((A_i, \A_{A_i}))$ \hfill$\COMMENT{\text{Plan gain-optimal policy } \pi_i \text{ for } A_i}$
	    \ENDFOR
	   % \STATE $((A'_1, g'_1), \ldots,(A'_k, g'_k)) \leftarrow \texttt{Filter}(((A_1, g_1), \ldots, (A_m, g_m)))$
	    \STATE Set $\pi_0 \leftarrow \texttt{PlanTransient}(((A_1, g_1), \ldots,(A_k, g_k)))$ \hfill$\COMMENT{\text{Plan shortest paths policy } \pi_0 \text{ to } \cup_{i=1}^k A_i}$
	\RETURN $\pi = \cup_{i=0}^k \pi_i$
	\end{algorithmic}
	\end{small}
\end{algorithm}
\end{minipage}

\textbf{Accepting End Components.} After sampling each state-action pair $\phi_{\texttt{AEC}}(\beta) = \frac{5}{\beta} \log(\frac{175 |\SState|^2 |A|}{\delta} ) = \Omega(\frac{1}{\beta})$ times, we can compute all of the maximal end components using Algorithm 47 from \cite{modelchecking}. Among these maximal end components, we remove the ones that are not accepting, which amounts to checking if EC $A_i$ contains a state in $\SState^\ast$. This concludes the preprocessing step of Line 3 in Algo \ref{algo:main}.


% The $\texttt{Sampler}$ function adds more samples to each state-action pair $(s,a)$, thereby refining $\mathcal{P}$.

% \begin{minipage}{.48 \textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{$\texttt{PlanRecurrent}$ ($\texttt{PR}$) } 
% 	\label{algo:AEC}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE End component $(A, \A_A)$
% 	    \STATE Set $\rho \leftarrow 2 \psi(\phi_{\texttt{AEC}}(\beta))$ \hfill$\COMMENT{\rho \sim \|P - \tilde{P}\|^{-1}_1}$
% 	    \REPEAT
% 	    \STATE Set $\rho \leftarrow \frac{\rho}{2}$
% 	   % \STATE Sample $\texttt{Sampler}(\phi_{\texttt{PR}}(\rho), A)$
% 	    \vspace{6pt}
	    
% 	    \quad $\COMMENT{\textit{Drive } \tilde{P} \to P}$
% 	    \STATE Sample $\phi_{\texttt{PR}}(\rho)$ times in $A \times \A_A$
% 	    \vspace{6pt}
	    
% 	    \quad $\COMMENT{\textit{(Relative) VI}}$
% 	    \STATE $v', v, \tilde{P} \leftarrow \texttt{VI}(\Bellman_{\texttt{PR}}, d_{\texttt{PR}}, \epsilon_{\texttt{PR}}, A, \{\}, 0)$ 
% 	    \vspace{6pt}
	    
% 	\UNTIL{$\rho > \frac{\epsilon_{\texttt{PR}} (1 - \tau_1(\tilde{P}))}{|A| c_{\max}}$ \hfill$\COMMENT{\|P - \tilde{P}\|_1 \textit{ small} }$}
% 	\smallskip
% 	\STATE Set policy $\pi \leftarrow \eta$-greedy policy w.r.t $v'$
% 	\STATE Set gain $g_\pi \leftarrow \frac{1}{2}\left(\max(v' - v) + \min(v'-v)\right)$
	
% 	\RETURN $\pi, g_\pi$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{$\texttt{PlanRecurrent}$ ($\texttt{PR}$) } 
% 	\label{algo:AEC}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE End component $(A, \A_A)$
% 	    \STATE Set $\rho = 2 \psi(\phi_{\texttt{AEC}}(\beta))$
% 	    \WHILE{True}
% 	    \STATE Set $\rho \leftarrow \frac{\rho}{2}$
% 	   % \STATE Sample $\texttt{Sampler}(\phi_{\texttt{PR}}(\rho), A)$
% 	    \STATE Sample $\phi_{\texttt{PR}}(\rho)$ times in $A \times \A_A$ 
% 	    \STATE $v', v, \tilde{P} \leftarrow \texttt{VI}(\Bellman_{\texttt{PR}}, d_{\texttt{PR}}, \epsilon, A, \{\}, 0)$
% 	    \STATE If $\rho > \frac{\epsilon (1 - \tau_1(\tilde{P}))}{|A| c_{\max}}$: \textbf{break}
% 	   % \STATE Set $\rho \leftarrow \frac{\rho}{2}$
% 	    \ENDWHILE
% 	\STATE Set $\pi = \eta$-greedy policy w.r.t $v'$
% 	\STATE $g_\pi = \frac{1}{2}\left(\max(v' - v) + \min(v'-v)\right)$
% 	\RETURN $\pi, g_\pi$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \hfill

\textbf{PlanRecurrent.} To plan in each accepting end component $(A, \A_A)$, we apply relative value iteration ($\texttt{VI}$, see App \ref{app:aditional_algorithms}, Algo \ref{algo:VI}) to the optimistic average-cost bellman operator:
\begin{wrapfigure}{l}{0.5\textwidth}
\vspace{-0.55cm}
\begin{minipage}{.48\textwidth}
\begin{algorithm}[H]
	\begin{small}
	%\renewcommand{\thealgorithm}{}
	\caption{$\texttt{PlanRecurrent}$ ($\texttt{PR}$) } 
	\label{algo:plan_recurrent}
	\begin{algorithmic}[1]
	    \REQUIRE End component $(A, \A_A)$
	    \STATE Set $\rho \leftarrow 2 \psi(\phi_{\texttt{AEC}}(\beta))$ \hfill$\COMMENT{\rho \sim \|P - \tilde{P}\|^{-1}_1}$
	    \REPEAT
	    \STATE Set $\rho \leftarrow \frac{\rho}{2}$
	   % \STATE Sample $\texttt{Sampler}(\phi_{\texttt{PR}}(\rho), A)$
	    \vspace{6pt}
	    
	    \quad $\COMMENT{\textit{Drive } \widehat{P} \to P}$
	    \STATE Sample $\psi^{-1}(\rho)$ times in $A \times \A_A$
	    \vspace{6pt}
	    
	    \quad $\COMMENT{\textit{(Relative) VI}}$
	    \STATE $v', v, \tilde{P} \leftarrow \texttt{VI}(\Bellman_{\texttt{PR}}, d_{\texttt{PR}}, \epsilon_{\texttt{PR}})$ 
	    \vspace{6pt}
	    
	\UNTIL{$\rho > \frac{\epsilon_{\texttt{PR}} (1 - \tau_1(\tilde{P}))}{|A| c_{\max}}$ \hfill$\COMMENT{\|P - \tilde{P}\|_1 \textit{ small} }$}
	\smallskip
	\STATE Set policy $\pi \leftarrow \eta$-greedy policy w.r.t $v'$
	\STATE Set gain $g_\pi \leftarrow \frac{1}{2}\left(\max(v' - v) + \min(v'-v)\right)$
	
	\RETURN $\pi, g_\pi$
	\end{algorithmic}
	\end{small}
\end{algorithm}
\end{minipage}
\vspace{-1.0cm}
\end{wrapfigure}
\begin{equation}
\begin{split}
    \label{eq:bellman_avg}
    \Bellman_{\texttt{PR}} v(s) = \min_{a \in \A_A(s)} \big(&\mathcal{C}(s,a) + \alpha \min_{p \in \mathcal{P}(s,a)} p^T v \big) \\
    &+ (1-\alpha) v(s) \quad \forall s \in A
\end{split}
\end{equation} 
where $\alpha \in (0,1)$ is an arbitrary aperiodicity transform coefficient, necessary for technical reasons but does not affect the gain of the greedy policy with respect to $v$. For properly chosen $\eta$ (Lemma \ref{lem:eta_greedy_approx}), the $\eta$-greedy policy (which we denote $\pi_\eta$) with respect to the solution of the Bellman operator $\Bellman_{\texttt{PR}}$ makes $A$ recurrent and the gain $g_{\pi_\eta}$ is close to $g_{\pi}$, where $\pi$ is the greedy policy. In practice $\eta$ can be chosen arbitrarily close to $1$.
Thus, LTL spec satisfaction conditioned on reaching $A$ is probability $1$.

% Essentially, $\alpha \neq 0$ implies that we are considering $P \in \mathcal{P}$ with $\alpha$ probability of self-loops $P(s,a,s) = \alpha$, aperiodic. 


% The policy returned by this algorithm will be sampling all actions with strictly positive probability inducing an ergoidic markov chain from $(A, \A_A)$. Thus, LTL spec satisfaction conditioned on reaching $A$ is probability $1$.



% needed (needed for technical reasons) until $d_{\texttt{PR}}(v_{n+1}, v_n) = \max_{s \in A}(v_{n+1}(s) - v_n(s)) - \min_{s \in A}(v_{n+1}(s) - v_n(s)) < \epsilon_{\texttt{PR}} \equiv \frac{\epsilon}{200}.$

For VI, we use the termination condition $d_{\texttt{PR}}(v_{n+1}, v_n) = \max_{s \in A}(v_{n+1}(s) - v_n(s)) - \min_{s \in A}(v_{n+1}(s) - v_n(s)) < \epsilon_{\texttt{PR}} \equiv \frac{2\epsilon}{3}.$
It is well known that relative value iteration is more stable than standard value iteration for calculating average-cost optimal policies, so we shift each entry of 
$v_n$ by the value of the first entry 
$v_n(0)$ \cite{bertsekas2011dynamic}. 

The algorithm returns the average cost $g_\pi$ of policy $\pi$ when we have enough samples for each state-action pair in $(A, \A_A)$ to verify that
\begin{equation*}
    n > \psi^{-1}\left( \frac{\epsilon_{\texttt{PR}} (1 - \Delta(\tilde{P}_\pi))}{|A| c_{\max}} \right) \quad \text{where }  \Delta(\tilde{P}_\pi) = \frac{1}{2} \max_{ij} \sum_{k} |\tilde{p}_{ik} - \tilde{p}_{jk}|
\end{equation*}
Here $\Delta(\tilde{P}_\pi)$ is an easily computable measure on the ergodicity of a markov chain $\tilde{P}_\pi$ \cite{cho2001ergodicity}. We track $\psi(n)$ (recall Def \ref{def:high_prob_event}) via a variable $\rho$ and sample $\psi^{-1}(\rho) \approx \frac{1}{\rho^2}$ (see Lemma \ref{lem:samples_req}) samples from each state-action pair in $(A, \A_A)$. We halve $\rho$ each iteration and convergence is guaranteed because $\rho$ will never fall below some unknown constant $\frac{\epsilon_{\texttt{PR}} (1- \bar{\Delta}_A)}{2|A|c_{\max}}$ (see Lem \ref{lem:simulation_avg}). We have to do the halving trick because we do not assume we know $\bar{\Delta}_A$.

\begin{restatable}[\texttt{PlanRecurrent} Convergence + Correctness]{prop}{gainConvCorrectness}
% \begin{prop}[Convergence + Correctness, Informal]
\label{prop:plan_recurrent}
Denote the gain-optimal policy in AEC $(A, \A)$ as $\pi_A$. Algorithm \ref{algo:plan_recurrent} terminates after a logarithmic number of repeats, when at worst $n \geq \Omega(\frac{|A|^2c_{\max}^2}{\epsilon_{\texttt{PR}}^2 (1- \bar{\Delta}_A)^2})$ samples have been collected for each state-action pair in $(A, \A_A)$. The $\eta$-greedy policy $\pi_{\eta}$ with respect to $v'$ (Line 5 of Alg \ref{algo:plan_recurrent}), the value function after VI, is both near-gain and probability optimal:
\begin{equation*}
    \|g_{\pi_{\eta}} - g_{\pi_A} \| < \epsilon, \quad \Prob{\pi_{\eta} \models \varphi | s_0 \in A} = 1
\end{equation*}
\end{restatable}

% We track a variable $\rho = \max_{s,a,s' \in A \times \A_A \times A, \tilde{P} \in \mathcal{P}} \|P(s,a,s') - \tilde{P}(s,a,s')\|_1 \leq \psi(n)$ where $n$ is the number of times the $(s,a) \in A \times \A_A$ has been sampled. As the number of samples increase, $\psi(n)$ decreases. We can calculate the number of samples necessary to achieve an error of $\rho$ as $ n = \psi^{-1}(\rho)$ (see \ref{lem:samples_req}).


\begin{rem}
For ease of exposition, we assume that there do not exist any probability $1$ paths between components $A_i$ and $A_j$. By this assumption, leaving an end component should have strictly less probability of satisfying the specification. In the presence of these paths, we'd have to filter out the higher gain components. This adds some computational complexity, but does not require more samples. We handle this case in a modified algorithm (See Appendix \ref{app:sec:filter_algo}).
\end{rem}

% \textbf{Filter} If there is a probability $1$ path achievable between two end components $A_i$ and $A_j$ with gains $g_i < g_j$, then the optimal gain policy should prefer $g_i$. Hence, we have an intermediate step to remove the sub-optimal AEC. To calculate the probability of paths to some end component $A_i$ we leverage the optimistic bellman operator:
% \begin{equation*}
%     \Bellman_{\texttt{F}} v(s) = \min_{a \in \A_A(s)}  \min_{p \in \mathcal{P}(s,a)}p^T v \quad s\in \SState
% \end{equation*}
% and $v(s) = 1$ for $s \in A_i$.
% $\texttt{VI}$ converges when $d_{\texttt{F}}(v_{n+1}, v_n) = \|v_{n+1} - v_n\|_1$ is sufficiently small. If $v(s) = 1$ for any $s \in A_j$ for $j \neq i$ and $g_j > g_i$ then there is a policy that can get from $A_i$ to $A_j$ and achieve lower gain, which is preferable. So we remove $A_j$ from our allowable end components.

% This procedure can be viewed as a stochastic shortest path problem \cite{}. For each round, the target states are $s \in A_i$ with terminal cost $1$ and intermediate costs $0$. 

\textbf{PlanTransient} This is the SSP reduction step. 
% Similar to $\texttt{Filter}$, this procedure can be also be viewed as a stochastic shortest path problem. For each round, the target states are any state within an AEC and the terminal cost is the gain of that state with respect to the policy calculated for that AEC.
To calculate the highest probability, lowest cost path to the end components we leverage the optimistic bellman operator:
\begin{equation*}
    \label{eq:bellman_transient}
    \Bellman_{\texttt{PT}} v(s) = \min\left\{\min_{a \in \A_A(s)} \left( \mathcal{C}(s,a) + \min_{p \in \mathcal{P}(s,a)}p^T v \right), \bar{V}\right\} \quad s\in \SState
\end{equation*}
and $v(s) = \lambda g_i$ for $s \in A_i$, the states we want to reach. 
% \begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-0.55cm}
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{$\texttt{PlanTransient}$ ($\texttt{PT}$) } 
% 	\label{algo:plan_transient}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE EC and gains $E=((A_1, g_1),\ldots,(A_k, g_k))$
% 	    \STATE Set $\bar{v} = 1$ \hfill$\COMMENT{\textit{a guess of }\|V\|_\infty}$
% 	    \STATE Set $V_T(s) = \lambda g_i$ for $s \in S_i$ \hfill$\COMMENT{\textit{Terminal costs}}$
% 	    \REPEAT
% 	    \STATE Set $\bar{v} \leftarrow 2 \bar{v}$
% 	   % \STATE Sample $\texttt{Sampler}(\phi_{\texttt{PT}}(\rho), \SState \setminus \cup_{i=1}^k A_i)$
% 	   \vspace{6pt}
	    
% 	    \quad $\COMMENT{\textit{Drive } \tilde{P} \to P}$
% 	    \STATE Sample $\phi_{\texttt{PT}}(\bar{v})$ times in $(\SState \setminus \cup A_i) \times \A$ 
% 	   %$\COMMENT{\text{Drive } \tilde{P} \to P}$
% 	   \vspace{6pt}
	    
% 	    \quad $\COMMENT{\textit{(SSP) VI}}$
% 	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{PT}}, d_{\texttt{PT}}, \epsilon_{\texttt{PT}}, \SState, \cup A_i, V_T)$
% 	    \vspace{6pt}
	    
% 	    \UNTIL{$\|v'\|_\infty < \bar{v}$}
% 	\STATE Set $\pi \leftarrow $greedy policy w.r.t $v'$
% 	\RETURN $\pi$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% % \vspace{-1.0cm}
% \end{wrapfigure}
\begin{wrapfigure}{l}{0.5\textwidth}
\vspace{-0.55cm}
\begin{minipage}{.48\textwidth}
\begin{algorithm}[H]
	\begin{small}
	%\renewcommand{\thealgorithm}{}
	\caption{$\texttt{PlanTransient}$ ($\texttt{PT}$) } 
	\label{algo:plan_transient}
	\begin{algorithmic}[1]
	    \REQUIRE EC and gains $E=((A_1, g_1),\ldots,(A_k, g_k))$
	    \STATE Set $V_T(s) = \lambda g_i$ for $s \in A_i$ \hfill$\COMMENT{\textit{Terminal costs}}$
	   % \REPEAT
	   % \STATE Set $\bar{v} \leftarrow 2 \bar{v}$
	   % \STATE Sample $\texttt{Sampler}(\phi_{\texttt{PT}}(\rho), \SState \setminus \cup_{i=1}^k A_i)$
	   %\vspace{6pt}
	    
	    \quad $\COMMENT{\textit{Drive } \widehat{P} \to P}$
	    \STATE Sample $\phi_{\texttt{PT}}(\bar{V})$ times in $(\SState \setminus \cup A_i) \times \A$ 
	   %$\COMMENT{\text{Drive } \tilde{P} \to P}$
	   \vspace{6pt}
	    
	    \quad $\COMMENT{\textit{(SSP) VI}}$
	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{PT}}, d_{\texttt{PT}}, \epsilon_{\texttt{PT}}, V_T)$
	    \vspace{6pt}
	    
	   % \UNTIL{$\|v'\|_\infty < \bar{v}$}
	\STATE Set $\pi \leftarrow $greedy policy w.r.t $v'$
	\RETURN $\pi$
	\end{algorithmic}
	\end{small}
\end{algorithm}
\end{minipage}
\vspace{-.5cm}
\end{wrapfigure}
Since rejecting components are possible, then we must bound $\|v\|_\infty < \bar{V}$ to prevent $v$ from blowing up. It was shown in \cite{Kolobov2012DeadEnd} that there exists, but not how to find, a $\bar{V}$ such that $\pi$ will reach the target states (in this case, the accepting components) first with highest probability and then with lowest cost. We show how to select $\bar{V}$ in Prop \ref{prop:J}. $\texttt{VI}$ converges when $d_{\texttt{PT}}(v_{n+1}, v_n) = \|v_{n+1} - v_n\|_1 < \epsilon_{\texttt{PT}} \equiv \frac{c_{\min} \epsilon}{4 \bar{V}}$. The number of samples required is $\phi_{\texttt{PT}}(\bar{V}) = \psi^{-1}\left(\frac{c_{\min} \epsilon }{14 |\SState \setminus \cup_{i=1}^k A_i| \bar{V}^2}\right)$, leading to a guarantee:
\begin{restatable}[\texttt{PlanTransient} Convergence \& Correctness]{prop}{transientConvCorrectness}
\label{prop:plan_transient}
% \begin{prop}[Convergence + Correctness, Informal]
Denote the value-optimal and probability optimal policy as $\pi^\ast$. Algorithm \ref{algo:plan_transient} after at worst $n \geq \Omega(\frac{|\SState \setminus \cup_{i=1}^k A_i|^2 \bar{V}^4}{c_{\min}^2 \epsilon^2 })$ samples have been collected for each state-action pair in $(\SState \setminus \cup_{i=1}^k A_i) \times \A$. The greedy policy $\pi$ with respect to $v'$ (Line 3 of Alg \ref{algo:plan_transient}), the value function after VI, is both cost and probability optimal:
\begin{equation*}
    \|V_{\pi} - V_{\pi^\ast} \| < \epsilon, \quad \Prob{\pi \text{ reaches } \cup_{i=1}^k A_i} = \Prob{\pi^\ast \text{ reaches } \cup_{i=1}^k A_i}
\end{equation*}
\end{restatable}



% The algorithm returns the highest prob and lowest cost policy $\pi$ when we have enough samples for each state-action pair in $\SState \setminus \cup_{i=1}^k A_i$ to verify that
% \begin{equation*}
%     \|v_{n+1}\|_\infty < \rho,
% \end{equation*}
% where $\rho$ doubles every iteration. The greedy policy with respect to $v_{n+1}$ is then $\epsilon$-optimal. Since rejecting components are possible, then we must bound $\|v\|_\infty < \bar{V}$ to prevent $v$ from blowing up. 



==> old_sec-background.tex <==
\section{Background}\label{sec:problem_formulation}

An atomic proposition is a statement that takes on a truth value. The set of all atomic propositions is given by $\text{AP}$. An alphabet is $\Sigma = 2^{\text{AP}}$. For example, if $\text{AP} = \{a, b\}$ then $\Sigma = \{\{\}, \{a\}, \{b\}, \{a,b\}\}$.

\subsection{MDPs with Labelled State Spaces}

We assume that the environment follows the finite Markov Decision Process (MDP) framework given by the tuple $\M = (\SState^\M, \A^\M, P^\M, \Cost^\M, d_0^\M, L)$ consisting of (i) a finite state $\SState^\M$, (ii) a finite action space $\A^\M$, (iii)
an \textit{\textbf{unknown}} transition function $P^\M : \SState^\M \times \A^\M \to \Delta(\SState^\M)$, (iv)
a cost function $\Cost : \SState^\M \times \A^\M \to \Delta([\cmin, \cmax])$, (v) an initial state distribution $d_0 \in \Delta(\SState^\M)$, and (vi) a labelling function $L: \SState^\M \to \Sigma$. We take $\A^\M(s)$ to be the set of available actions in state $s$.

% A (stochastic) policy $\pi: \SState^\M \to \Delta(\A^\M)$ determines a distribution $\Tau_{\pi}$ over trajectories of the form 
% $s0, a0, r0, s1, a1, r1, . . . , where s0 ∼ d0, at ∼ π(st), rt ∼
% R(st, at), and st+1 ∼ P(st, at) 

\begin{rem}
The cost function $\Cost^\M$ does not encode information about the task. Rather, it serves as a way to discriminate amongst policies.
\end{rem}

Unlike traditional MDPs, $\M$ is endowed with a labelling function $L$ which returns the AP that are true in that state. A \textit{run} in $\M$ is a sequence of transitions given by $\tau = (s_0,s_1,\ldots)$.
% and a \textit{word} is an infinite sequence of labels $L(\tau) = (L(s_0),L(s_1),\ldots)$. 

\subsection{Policies and Decomposition}

Let $\Pi = \{ \pi(s) \in \Delta(\A(s)) \; \forall s \in \SState \}$ be a set of (stochastic) Markovian policies defined over some state space $\SState$. It is often convenient to focus on $\pi$ restricted to a set of states $X \subseteq \SState$, and call this ``$\pi$ in $X$''. A policy $\pi$ can be thought of as a  combination of the (partial) policies $\pi_i$ where each $\pi_i$ acts only on $\SState_i$ and the sets $\SState_i$ partition $\SState$, mutually exclusively. We denote this as $\pi = \cup_{i=1}^k \pi_i$.

\subsection{Linear Temporal Logic (LTL)}

We cover the scope of LTL relevant to understand the examples and theory in this work. 
\begin{defn}[LTL Specification, $\varphi$]
An LTL specification $\varphi$ is the entire description of the task and is constructed from composition of atomic propositions with the logical connectives not ($\lnot$), and ($\&$) and implies
($\rightarrow$), together with the temporal operators, next $(X)$, always/globally ($G$), eventually ($F$) and until ($U$).
\end{defn}

For example, for atomic propositions $a,b$, we can create the tasks/specifications: safety ($\lnot b$), reachability ($F g$),
stability ($FGg$), response ($a \rightarrow F b$), progress $(a \;\&\; F X b)$. Complicated expressions such as ``track a trajectory while avoiding undesirable locations'' can be
obtained through proper composition of simpler safety, reachability and progress formulas. For a more formal and comprehensive overview of the syntax and semantics of LTL, we encourage the reader to see \cite{modelchecking}.

An LTL specification $\varphi$ has a corresponding LDBA $\mathcal{B}_\varphi$ \cite{ldba}, modelling the progression of satisfying the specification. While $\B_\varphi$ is a specific to $\varphi$, for ease of notation we drop the dependence when unambiguous.

\begin{defn}(Limit Deterministic B\"uchi Automaton, LDBA \cite{ldba})
A \textbf{\textit{LDBA}} is a tuple $\mathcal{B} = (\SState^\B, \Sigma, P^\B, \SState^\mathcal{B \ast}, s^\B_0)$ consisting of (i) a finite set of states $\SState^\B$, (ii) a finite alphabet $\Sigma = 2^{\text{AP}}$  where AP are atomic prepositions, (iii) a transition function $P^\B : \SState^\B \times \Sigma \to 2^{\SState^\B}$, (iv) a set of accepting states $\SState^\mathcal{B \ast} \subseteq \SState^\B$, and (v) an initial state $s^\B_0$. Further, there exists a mutually exclusive partitioning of $\SState^\B = \SState^\B_D \cup \SState^\B_{ND}$ such that $\SState^\mathcal{B \ast} \subseteq \SState^\B_D$, and for $s \in S^\B_D, a \in \Sigma$ then $P^\B(s, a) \subseteq \SState^\B_D$ and $|P^\B(s, a)| = 1$. There is a (possibly empty) set $\A_\B(s)$ of special transitions in $s \in \SState^\B_{ND}$ that lead to states in $\SState^\B_{D}$. These transitions may be taken at any time, without needing to follow $P^\B$, and amount to a ``guess'' that we've entered the deterministic part of the automaton. A \textit{path} $\sigma = (s_0, s_1, \ldots)$ is a sequence of transitions in $\mathcal{B}$.  $\mathcal{B}$ \textbf{accepts} a path $\sigma$ if there exists some state $s \in \SState^\mathcal{B \ast}$ in the path that is visited infinitely often.
% In other words, the accepting part of the LDBA automaton is deterministic and invariant. The transition between $Q_{ND}$ and $Q_{D}$ is done via $\alpha$ transitions, which amounts to a ``guess'' that the automata has entered the deterministic part of the state space. Let $\A_{\mathcal{L}}(q)$ be the set of $\alpha$ transitions possible in $q \in Q_{ND} \subset \SState^\B$.
\end{defn}

\subsection{LTL Satisfaction}

\clv{Add sentence referencing Problem Formulation} There is a tight connection between runs in $\M$ inducing runs in $\B$.
Specifically, starting in $s_0^{\B}$ then $s_i^\B \sim P^\B(s_{i-1}^{\B}, L(s_{i-1}^\M))$ where $\tau^\M = (s_0^\M, s_{1}^\M,\ldots)$ is a run in $\M$. It is often convenient to think of the interaction between $\M$ and $\B$ as a synchronized product-MDP.

\begin{defn}(Product MDP)
The product MDP $\mathcal{X}_{\M, \B} = (\SState, \A, P, \Cost, d_0, L, \SState^{\ast})$ is an MDP with $\SState = \SState^\M \times \SState^\B$, $\A = \A^{\M} \cup \A^{\B}$, $\Cost((m, b),a) = \Cost^{\M}(m,a)$ if $a \in A^{\M}(m)$ otherwise $0$, $d_0 = d_0^\M \times \{s_0^\B\}$, $L((m,b)) = L^\M(m)$, $S^\ast = \{(\cdot, b) \in \SState | b \in \SState^{\B \ast}\}$ is the set of accepting states, and $P: \SState \times \A \to \Delta(\SState)$ taking the form
\begin{equation*}
    P((m, b),a,(m', b')) = 
    \begin{cases} 
    P^{\M}(m,a,m') P^{\B}(b,L(m'),b'), 
    &a \in A^{\M}(m) \\
    P^{\B}(b,L(m'),b'), &m=m', a \in  A^{\B}(b) \\
    0, &\text{otherwise}
    \end{cases}
\end{equation*} 
\end{defn}

A run $\tau = (s_0, s_1, \ldots) = ((s_0^\M, s_0^\B), (s_1^\M, s_1^\B), \ldots)$ in $\X$ is accepting (accepted) iff the run $(s_0^\B,s_1^\B,\ldots)$ in $\B$ is accepting iff there exists some $s \in \SState^\ast$ visited infinitely often. This leads us to the following definition of LTL satisfaction:

\begin{defn}(Satisfaction, Run)
A run $\tau$ in $\X$ \textit{satisfies} the LTL specification $\varphi$ if it is accepted.
\end{defn}

A policy $\pi \in \Pi$ induces a probability distribution over runs $\tau$ in $\X$. In fact, $\pi$ with transition function $P$ induces a discrete-time markov chain and separates the state space $\SState = T \cup R_1 \cup \cdots \cup R_k$ into a set of transient states $T$, visited finitely with probability $1$, and recurrent states $R_i$, trapping and visited infinitely often with probability $1$. Hence, all policies reach some $R_i$ and stay there forever. If a run reaches $R_i$ and $R_i$ contains an accepting state then the run is accepted and $\varphi$ is satisfied. This leads us to the definition of a policy satisfying a specification.

\begin{defn}(Satisfaction, Policy)
A policy $\pi \in \Pi$ \textit{satisfies} the LTL specification $\varphi$ with probability $\mathbb{P}(\pi \models \varphi) = \E_{\tau \sim \Tau^P_\pi}[1_{\tau \models \varphi}] = \sum_{i=1}^k \mathbb{P}(\tau \text{ reaches } R_i) * \mathbf{1}_{R_i \cap \SState^\ast \neq \varnothing}$. Here, $\mathbf{1}_{X}$ is an indicator variable which is $1$ when $X$ is true, otherwise $0$. $\Tau^P_{\pi}$ is the set of trajectories induced by $\pi$ in $\X$ with transition function $P$.
\end{defn}




% Suppose we endow $\mathcal{M}$ with a labelling function $L: \SState^\M \to \Sigma$. Intuitively, $L(s)$ is checking which AP are true in state $s \in \SState^\M$. An LTL specification $\varphi$ has a corresponding LDBA $\mathcal{B}_\varphi$ that accepts only if $\varphi$ is satisfied. 


% It is well known that an LTL specification can be reformulated as an automaton that keeps track of the progression towards satisfying the specification \cite{}. One of the more recent ones is known as a Limit Deterministic B\"uchi Automaton (LDBA). The LDBA consists of a set of states, deterministic and non-deterministic transitions, and set of accepting states. \textit{The specification is satisfied if the set of accepting states is visited infinitely often.}

% Formally, an LDBA $\mathcal{L} = (\SState^\B, \Sigma, F, P^\B)$ is given by $\SState^\B$ a finite set of states, $\Sigma = 2^{\text{AP}}$ is a finite alphabet where AP are atomic prepositions, $F \subseteq \SState^\B$ is the set of accepting states and $P^\B : \SState^\B \times \Sigma \to 2^{\SState^\B}$. Further, $Q = Q_D \cup Q_{ND}$ can be partitioned into mutually exclusive sets such that $F \subseteq Q_D$, and for $q \in Q_D, a \in 2^{\text{AP}}$ then $P^\B(q, a) \subseteq Q_D$ and $|P^\B(q, a)| = 1$. In other words, the accepting part of the LDBA automaton is deterministic and invariant. The transition between $Q_{ND}$ and $Q_{D}$ is done via $\alpha$ transitions, which amounts to a ``guess'' that the automata has entered the deterministic part of the state space. Let $\A_{\mathcal{L}}(q)$ be the set of $\alpha$ transitions possible in $q \in Q_{ND} \subset \SState^\B$.

\subsection{Graph Theory}

\clv{combine with 4.1} Throughout our analysis, we will rely on the idea of end components. An end component is a sub-MDP of a larger MDP that is probabilistically closed. Intuitively, it is a recurrent, inescapable set of states when restricted to a certain action set.

\begin{defn}(End Component)\label{def:end_component} Consider some MDP $(\SState, \A, P, \mathcal{C}, d_0)$. An end component $(E, \A_E)$ is a set of states $E \subseteq \SState$ and acceptable actions $\A_E(s) \subseteq \A(s)$ (where $s \in E$) such that $\{s' | \exists s \in E, a \in A_E(s) \text{ s.t. } P(s,a, s') > 0 \} \subseteq E$. Furthermore, $(E, \A_E)$ is strongly connected:  any two states in $E$ is reachable from one another by means of actions in $A_E$. We say an end component $(E, \A_E)$ is \textit{maximal} if it is not contained within a larger end component $(E', \A_{E'})$, ie. $\nexists (E, \A_{E'})$, end component, where $E \subseteq E', \A_E(s) \subseteq \A_{E'}(s)$ for each $s \in A$.
\end{defn}


% After we have the structure of the graph, we can identify the recurring components. These components, otherwise known as end components \cite{modelchecking}, are a set of states and actions $(A, \A_A)$ that is probabilistically closed. That is, if you take an action $a \in \A_A$ in state $s \in A$ then the next state is still in $A$, i.e $\{s' | P(s,a, s') > 0 \} \subseteq A$. Furthermore, we require $A$ to be strongly-connected, that any two states in $A$ is reachable from one another by means of actions in $\A$. We say an end component $(A, \A_A)$ is maximal if it is not contained within a larger end component $(B, \A_B)$, ie. $\nexists (B, \A_B)$ where $A \subseteq B, \A_A(s) \subseteq \A_B(s)$ for each $s \in A$.

% \subsection{Product Space}

% % We assume that the environment follows the discrete Markov Decision Process (MDP) framework given by the tuple $\mathcal{M} = (\SState^\M, \A^\M, P^\M, \Cost^\M)$ with $\SState^\M$ as the discrete state space, $\A^\M$ as the
% % discrete action space, $P^\M : \SState^\M \times \A^\M \to \Delta(\SState^\M)$ is the (unknown) transition function,
% % $\Cost : \SState^\M \times \A^\M \to \Delta([\cmin, \cmax])$ is the cost function. Note that the cost function $\Cost^\M$ does not encode information about the task.

% We combine the LDBA encoding the desired LTL specification with the MDP into the following product space $\mathcal{X} = (\SState, \A, L, P, \mathcal{C})$ where $(m, q) \in \SState = \SState^\M \times \SState^\B$, $\A(m, q) = \A_{\mathcal{M}} \cup \A_{\mathcal{L}}(q)$ are the actions available in product-state $s = (m, q) \in \SState$, $L: \SState_{\mathcal{M}} \to \Sigma$ the labelling function of the MDP, $P: \SState \times \A \to \Delta(\SState)$ the transition function that takes the form 
% \begin{equation*}
%     P((m,q),a,(m',q')) = 
%     \begin{cases} 
%     P_{\mathcal{M}}(m,a,m') P_{\mathcal{L}}(q,L(m'),q'), 
%     &a \in A_{\mathcal{M}}(m) \\
%     P_{\mathcal{L}}(q,L(m'),q'), &m=m', a \in  A_{\mathcal{L}}(q) \\
%     0, &\text{otherwise}
%     \end{cases}
% \end{equation*}
% and $\Cost((m, q),a) = \Cost_{\mathcal{M}}(m,a)$ if $a \in A_{\mathcal{M}}(m)$ otherwise $\Cost((m, q),a) = 0$, is the cost function.


==> sec-problem.tex <==
\section{Problem Formulation}\label{sec:problem_formulation}

We begin with some definitions to understand the problem statement. An atomic proposition is a statement that takes on a truth value. The set of all atomic propositions is given by $\text{AP}$. An alphabet is $\Sigma = 2^{\text{AP}}$. For example, if $\text{AP} = \{a, b\}$ then $\Sigma = \{\{\}, \{a\}, \{b\}, \{a,b\}\}$. We consider the policy space of (stochastic) Markovian policies, denoted $\Pi$.

\subsection{MDPs with Labelled State Spaces} 

We assume that the environment follows the finite Markov Decision Process (MDP) framework given by the tuple $\M = (\SState^\M, \A^\M, P^\M, \Cost^\M, d_0^\M, L^{\mathcal{M}})$ consisting of (i) a finite state $\SState^\M$, (ii) a finite action space $\A^\M$, (iii)
an \textit{\textbf{unknown}} transition function $P^\M : \SState^\M \times \A^\M \to \Delta(\SState^\M)$, (iv)
a cost function $\Cost : \SState^\M \times \A^\M \to \Delta([\cmin, \cmax])$, (v) an initial state distribution $d_0 \in \Delta(\SState^\M)$, and (vi) a labelling function $L^{\mathcal{M}}: \SState^\M \to \Sigma$. We take $\A^\M(s)$ to be the set of available actions in state $s$. Unlike traditional MDPs, $\M$ is endowed with a labelling function $L^{\mathcal{M}}$ which returns the AP that are true in that state. A \textbf{run} in $\M$ is a sequence of transitions given by $\tau = (s_0,s_1,\ldots)$.


% and a \textit{word} is an infinite sequence of labels $L(\tau) = (L(s_0),L(s_1),\ldots)$. 

% A (stochastic) policy $\pi: \SState^\M \to \Delta(\A^\M)$ determines a distribution $\Tau_{\pi}$ over trajectories of the form 
% $s0, a0, r0, s1, a1, r1, . . . , where s0 ∼ d0, at ∼ π(st), rt ∼
% R(st, at), and st+1 ∼ P(st, at) 

% \begin{rem}
% The cost function $\Cost^\M$ does not encode information about the task. Rather, it serves as a way to discriminate amongst policies.
% \end{rem}

% Unlike traditional MDPs, $\M$ is endowed with a labelling function $L$ which returns the AP that are true in that state. A \textit{run} in $\M$ is a sequence of transitions given by $\tau = (s_0,s_1,\ldots)$.
% % and a \textit{word} is an infinite sequence of labels $L(\tau) = (L(s_0),L(s_1),\ldots)$. 

% \subsection{Policies and Decomposition}

% Let $\Pi = \{ \pi(s) \in \Delta(\A(s)) \; \forall s \in \SState \}$ be a set of (stochastic) Markovian policies defined over some state space $\SState$. It is often convenient to focus on $\pi$ restricted to a set of states $X \subseteq \SState$, and call this ``$\pi$ in $X$''. A policy $\pi$ can be thought of as a  combination of the (partial) policies $\pi_i$ where each $\pi_i$ acts only on $\SState_i$ and the sets $\SState_i$ partition $\SState$, mutually exclusively. We denote this as $\pi = \cup_{i=1}^k \pi_i$.

\textbf{\subsection{Linear Temporal Logic (LTL)}} We cover the scope of LTL relevant to understand the examples and theory in this work. For a more comprehensive overview of the syntax and semantics of LTL, we encourage the reader to see \cite{modelchecking}.

\begin{defn}[LTL Specification, $\varphi$]
An LTL specification $\varphi$ is the entire description of the task and is constructed from composition of atomic propositions with the logical connectives not ($\lnot$), and ($\&$) and implies
($\rightarrow$), together with the temporal operators, next $(X)$, always/globally ($G$), eventually ($F$) and until ($U$):
\begin{equation*}
    \varphi \equiv \text{true} \;|\; a \in AP \;|\; \varphi_1 \;\&\; \varphi_2 \;|\; \lnot \varphi \;|\; X \varphi \;|\; \varphi_1 U \varphi_2,
\end{equation*}
where the remaining connectives and operators are all derivatives.
\end{defn}

For example, for atomic propositions $a,b$, we can create the tasks/specifications: safety ($\lnot b$), reachability ($F g$),
stability ($FGg$), response ($a \rightarrow F b$), progress $(a \;\&\; F X b)$. Complicated expressions such as ``track a trajectory while avoiding undesirable locations'' can be
obtained through proper composition of simpler safety, reachability and progress formulas. 

\begin{defn}[Trajectory satisfaction, $\tau \models \varphi$]\label{def:traj_satisfaction} We say a run $\tau = (s_0,s_1,\ldots)$ in a (labelled) MDP satisfies specification $\varphi$, denoted $\tau \models \varphi$, by following recursive semantics:
\begin{minipage}{.4\linewidth}
\begin{align*}
\tau \models \begin{cases}
    true & \\
    a &\quad\text{iff } a \in L^{\mathcal{M}}(s_0), a \in AP  \\
    \varphi_1 \;\&\; \varphi_2 &\quad\text{iff } \tau \models \varphi_1 \text{ and }  \tau \models \varphi_2 \\
    % \lnot\varphi &\quad\text{iff } \tau \not\models \varphi \\
    % \tau \models X \varphi &\quad\text{iff } (s_1,\ldots) \models \varphi \\
    % \phi_1 U \phi_2 &\quad\text{iff } \exists j \geq 0,  (s_j,\ldots) \models \varphi_2 \text{ and } (s_i,\ldots) \models \varphi_1, \forall 0 \leq i < j \\
\end{cases}
\end{align*}
\end{minipage}%
\hfill
\begin{minipage}{.5\linewidth}
\begin{align*}
\begin{cases}
    % true & \\
    % a &\quad\text{iff } a \in L(s_0), a \in AP  \\
    % \varphi_1 \;\&\; \varphi_2 &\quad\text{iff } \tau \models \varphi_1 \text{ and }  \tau \models \varphi_2 \\
    \lnot\varphi &\quad\text{iff } \tau \not\models \varphi \\
    X \varphi &\quad\text{iff } (s_1,\ldots) \models \varphi \\
    \phi_1 U \phi_2 &\quad\text{iff } \exists j \geq 0,  (s_j,\ldots) \models \varphi_2 \\
    &\text{ and } (s_i,\ldots) \models \varphi_1, \forall 0 \leq i < j \\
\end{cases}
\end{align*}
\end{minipage}
\end{defn}

\begin{defn}(Policy Satisfaction, $\pi \models \varphi$)
A policy $\pi \in \Pi$ \textit{satisfies} the LTL specification $\varphi$ with probability $\Prob{\pi \models \varphi} = \E_{\tau \sim \Tau^{P}_\pi}[\mathbf{1}_{\tau \models \varphi}]$, where $T_{\pi}^{P}$ is the set of trajectories induced by $\pi$ in $\mathcal{M}$ with transition function $P$. Here, $\mathbf{1}_{X}$ is an indicator variable which is $1$ when $X$ is true, otherwise $0$.
\end{defn}


% An LTL specification $\varphi$ has a corresponding LDBA $\mathcal{B}_\varphi$ \cite{ldba}, modelling the progression of satisfying the specification. While $\B_\varphi$ is a specific to $\varphi$, for ease of notation we drop the dependence when unambiguous.

% \begin{defn}(Limit Deterministic B\"uchi Automaton, LDBA \cite{ldba})
% A \textbf{\textit{LDBA}} is a tuple $\mathcal{B} = (\SState^\B, \Sigma, P^\B, \SState^\mathcal{B \ast}, s^\B_0)$ consisting of (i) a finite set of states $\SState^\B$, (ii) a finite alphabet $\Sigma = 2^{\text{AP}}$  where AP are atomic prepositions, (iii) a transition function $P^\B : \SState^\B \times \Sigma \to 2^{\SState^\B}$, (iv) a set of accepting states $\SState^\mathcal{B \ast} \subseteq \SState^\B$, and (v) an initial state $s^\B_0$. Further, there exists a mutually exclusive partitioning of $\SState^\B = \SState^\B_D \cup \SState^\B_{ND}$ such that $\SState^\mathcal{B \ast} \subseteq \SState^\B_D$, and for $s \in S^\B_D, a \in \Sigma$ then $P^\B(s, a) \subseteq \SState^\B_D$ and $|P^\B(s, a)| = 1$. There is a (possibly empty) set $\A_\B(s)$ of special transitions in $s \in \SState^\B_{ND}$ that lead to states in $\SState^\B_{D}$. These transitions may be taken at any time, without needing to follow $P^\B$, and amount to a ``guess'' that we've entered the deterministic part of the automaton. A \textit{path} $\sigma = (s_0, s_1, \ldots)$ is a sequence of transitions in $\mathcal{B}$.  $\mathcal{B}$ \textbf{accepts} a path $\sigma$ if there exists some state $s \in \SState^\mathcal{B \ast}$ in the path that is visited infinitely often.
% % In other words, the accepting part of the LDBA automaton is deterministic and invariant. The transition between $Q_{ND}$ and $Q_{D}$ is done via $\alpha$ transitions, which amounts to a ``guess'' that the automata has entered the deterministic part of the state space. Let $\A_{\mathcal{L}}(q)$ be the set of $\alpha$ transitions possible in $q \in Q_{ND} \subset \SState^\B$.
% \end{defn}

% \subsection{LTL Satisfaction}

% \clv{Add sentence referencing Problem Formulation} There is a tight connection between runs in $\M$ inducing runs in $\B$.
% Specifically, starting in $s_0^{\B}$ then $s_i^\B \sim P^\B(s_{i-1}^{\B}, L(s_{i-1}^\M))$ where $\tau^\M = (s_0^\M, s_{1}^\M,\ldots)$ is a run in $\M$. It is often convenient to think of the interaction between $\M$ and $\B$ as a synchronized product-MDP.

% \begin{defn}(Product MDP)
% The product MDP $\mathcal{X}_{\M, \B} = (\SState, \A, P, \Cost, d_0, L, \SState^{\ast})$ is an MDP with $\SState = \SState^\M \times \SState^\B$, $\A = \A^{\M} \cup \A^{\B}$, $\Cost((m, b),a) = \Cost^{\M}(m,a)$ if $a \in A^{\M}(m)$ otherwise $0$, $d_0 = d_0^\M \times \{s_0^\B\}$, $L((m,b)) = L^\M(m)$, $S^\ast = \{(\cdot, b) \in \SState | b \in \SState^{\B \ast}\}$ is the set of accepting states, and $P: \SState \times \A \to \Delta(\SState)$ taking the form
% \begin{equation*}
%     P((m, b),a,(m', b')) = 
%     \begin{cases} 
%     P^{\M}(m,a,m') P^{\B}(b,L(m'),b'), 
%     &a \in A^{\M}(m) \\
%     P^{\B}(b,L(m'),b'), &m=m', a \in  A^{\B}(b) \\
%     0, &\text{otherwise}
%     \end{cases}
% \end{equation*} 
% \end{defn}

% A run $\tau = (s_0, s_1, \ldots) = ((s_0^\M, s_0^\B), (s_1^\M, s_1^\B), \ldots)$ in $\X$ is accepting (accepted) iff the run $(s_0^\B,s_1^\B,\ldots)$ in $\B$ is accepting iff there exists some $s \in \SState^\ast$ visited infinitely often. This leads us to the following definition of LTL satisfaction:

% \begin{defn}(Satisfaction, Run)
% A run $\tau$ in $\X$ \textit{satisfies} the LTL specification $\varphi$ if it is accepted.
% \end{defn}

% A policy $\pi \in \Pi$ induces a probability distribution over runs $\tau$ in $\X$. In fact, $\pi$ with transition function $P$ induces a discrete-time markov chain and separates the state space $\SState = T \cup R_1 \cup \cdots \cup R_k$ into a set of transient states $T$, visited finitely with probability $1$, and recurrent states $R_i$, trapping and visited infinitely often with probability $1$. Hence, all policies reach some $R_i$ and stay there forever. If a run reaches $R_i$ and $R_i$ contains an accepting state then the run is accepted and $\varphi$ is satisfied. This leads us to the definition of a policy satisfying a specification.

% \begin{defn}(Satisfaction, Policy)
% A policy $\pi \in \Pi$ \textit{satisfies} the LTL specification $\varphi$ with probability $\mathbb{P}(\pi \models \varphi) = \E_{\tau \sim \Tau^P_\pi}[1_{\tau \models \varphi}] = \sum_{i=1}^k \mathbb{P}(\tau \text{ reaches } R_i) * \mathbf{1}_{R_i \cap \SState^\ast \neq \varnothing}$. Here, $\mathbf{1}_{X}$ is an indicator variable which is $1$ when $X$ is true, otherwise $0$. $\Tau^P_{\pi}$ is the set of trajectories induced by $\pi$ in $\X$ with transition function $P$.
% \end{defn}




% Suppose we endow $\mathcal{M}$ with a labelling function $L: \SState^\M \to \Sigma$. Intuitively, $L(s)$ is checking which AP are true in state $s \in \SState^\M$. An LTL specification $\varphi$ has a corresponding LDBA $\mathcal{B}_\varphi$ that accepts only if $\varphi$ is satisfied. 


% It is well known that an LTL specification can be reformulated as an automaton that keeps track of the progression towards satisfying the specification \cite{}. One of the more recent ones is known as a Limit Deterministic B\"uchi Automaton (LDBA). The LDBA consists of a set of states, deterministic and non-deterministic transitions, and set of accepting states. \textit{The specification is satisfied if the set of accepting states is visited infinitely often.}

% Formally, an LDBA $\mathcal{L} = (\SState^\B, \Sigma, F, P^\B)$ is given by $\SState^\B$ a finite set of states, $\Sigma = 2^{\text{AP}}$ is a finite alphabet where AP are atomic prepositions, $F \subseteq \SState^\B$ is the set of accepting states and $P^\B : \SState^\B \times \Sigma \to 2^{\SState^\B}$. Further, $Q = Q_D \cup Q_{ND}$ can be partitioned into mutually exclusive sets such that $F \subseteq Q_D$, and for $q \in Q_D, a \in 2^{\text{AP}}$ then $P^\B(q, a) \subseteq Q_D$ and $|P^\B(q, a)| = 1$. In other words, the accepting part of the LDBA automaton is deterministic and invariant. The transition between $Q_{ND}$ and $Q_{D}$ is done via $\alpha$ transitions, which amounts to a ``guess'' that the automata has entered the deterministic part of the state space. Let $\A_{\mathcal{L}}(q)$ be the set of $\alpha$ transitions possible in $q \in Q_{ND} \subset \SState^\B$.

% \subsection{Graph Theory}

% \clv{combine with 4.1} Throughout our analysis, we will rely on the idea of end components. An end component is a sub-MDP of a larger MDP that is probabilistically closed. Intuitively, it is a recurrent, inescapable set of states when restricted to a certain action set.

% \begin{defn}(End Component)\label{def:end_component} Consider some MDP $(\SState, \A, P, \mathcal{C}, d_0)$. An end component $(E, \A_E)$ is a set of states $E \subseteq \SState$ and acceptable actions $\A_E(s) \subseteq \A(s)$ (where $s \in E$) such that $\{s' | \exists s \in E, a \in A_E(s) \text{ s.t. } P(s,a, s') > 0 \} \subseteq E$. Furthermore, $(E, \A_E)$ is strongly connected:  any two states in $E$ is reachable from one another by means of actions in $A_E$. We say an end component $(E, \A_E)$ is \textit{maximal} if it is not contained within a larger end component $(E', \A_{E'})$, ie. $\nexists (E, \A_{E'})$, end component, where $E \subseteq E', \A_E(s) \subseteq \A_{E'}(s)$ for each $s \in A$.
% \end{defn}


% After we have the structure of the graph, we can identify the recurring components. These components, otherwise known as end components \cite{modelchecking}, are a set of states and actions $(A, \A_A)$ that is probabilistically closed. That is, if you take an action $a \in \A_A$ in state $s \in A$ then the next state is still in $A$, i.e $\{s' | P(s,a, s') > 0 \} \subseteq A$. Furthermore, we require $A$ to be strongly-connected, that any two states in $A$ is reachable from one another by means of actions in $\A$. We say an end component $(A, \A_A)$ is maximal if it is not contained within a larger end component $(B, \A_B)$, ie. $\nexists (B, \A_B)$ where $A \subseteq B, \A_A(s) \subseteq \A_B(s)$ for each $s \in A$.

% \subsection{Product Space}

% % We assume that the environment follows the discrete Markov Decision Process (MDP) framework given by the tuple $\mathcal{M} = (\SState^\M, \A^\M, P^\M, \Cost^\M)$ with $\SState^\M$ as the discrete state space, $\A^\M$ as the
% % discrete action space, $P^\M : \SState^\M \times \A^\M \to \Delta(\SState^\M)$ is the (unknown) transition function,
% % $\Cost : \SState^\M \times \A^\M \to \Delta([\cmin, \cmax])$ is the cost function. Note that the cost function $\Cost^\M$ does not encode information about the task.

% We combine the LDBA encoding the desired LTL specification with the MDP into the following product space $\mathcal{X} = (\SState, \A, L, P, \mathcal{C})$ where $(m, q) \in \SState = \SState^\M \times \SState^\B$, $\A(m, q) = \A_{\mathcal{M}} \cup \A_{\mathcal{L}}(q)$ are the actions available in product-state $s = (m, q) \in \SState$, $L: \SState_{\mathcal{M}} \to \Sigma$ the labelling function of the MDP, $P: \SState \times \A \to \Delta(\SState)$ the transition function that takes the form 
% \begin{equation*}
%     P((m,q),a,(m',q')) = 
%     \begin{cases} 
%     P_{\mathcal{M}}(m,a,m') P_{\mathcal{L}}(q,L(m'),q'), 
%     &a \in A_{\mathcal{M}}(m) \\
%     P_{\mathcal{L}}(q,L(m'),q'), &m=m', a \in  A_{\mathcal{L}}(q) \\
%     0, &\text{otherwise}
%     \end{cases}
% \end{equation*}
% and $\Cost((m, q),a) = \Cost_{\mathcal{M}}(m,a)$ if $a \in A_{\mathcal{M}}(m)$ otherwise $\Cost((m, q),a) = 0$, is the cost function.



\subsection{Formulation}

% Together with $\mathcal{X}$, a deterministic Markovian policy $\pi(s) = a \in \A(s)$ induces a discrete-time Markov Chain (DTMC). Hence, for a fixed policy $\pi$,  we can partition $\SState = T \cup R_1 \cup \ldots \cup R_k$ where $T$ is a set of transient states and $R_i$ are sets of recurrent states \cite{}. Some $R_i$ must be reached because $T$ is transient, every state $s \in R_i$ will be visited infinitely often and the DTMC will never leave $R_i$. If the set $R_i$ contains states that are accepting in $\mathcal{L}$ then 

Our goal is to find a policy that simultaneously satisfies a given LTL specification with highest probability and is optimal respect to the cost function of the MDP. We define the gain (average-cost) and transient cost as
\begin{equation}\label{def:costs}
\begin{split}
g^P_\pi \equiv &\mathbb{E}_{\tau \sim \Tau^P_{\pi}} \left[ \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Cost(s_t, \pi(s_t)) \bigg| \tau \models \varphi \right], \quad J^P_\pi \equiv \mathbb{E}_{\tau \sim \Tau^P_{\pi}}\left[\sum_{t=0}^{\kappa_{\pi}} \Cost(s_t, \pi(s_t)) \bigg| \tau \models \varphi \right],
\end{split}
\end{equation}
% $\Tau^P_{\pi}$ is the set of trajectories induced by $\pi$ in $\X$ with transition function $P$.
where $\kappa_\pi$ is the first, unknown (hitting) time the trajectory $\tau$ leaves the transient states induced by $\pi$. Gain optimality for infinite horizon problems has a long history in RL \cite{bertsekas2011dynamic, puterman2014markov}.

For any $\lambda \geq 0$, the optimal policy is defined as
% \begin{equation}\label{eqn:gain_optimal_policies}
% \begin{split}
% \tilde{\Pi} = \min_{\pi \in \Pi} \; &\mathbb{E}_{\tau \sim \Tau_{\pi}}
% % \left[ \overbrace{\sum_{t=0}^{\kappa_\tau} \Cost(s_t, \pi(s_t))}^{\text{transient}} + \overbrace{\lim_{T \to \infty} \frac{1}{T-\kappa_\tau} \sum_{t=\kappa_\tau}^T \Cost(s_t, \pi(s_t))}^{\text{recurring}} \right] \\
% \left[ \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^{T-1} \Cost(s_t, \pi(s_t)) \right] (\equiv \min_{\pi \in \Pi} g_\pi)\\
% &\text{ s.t. } \Prob{\pi \models \varphi} \text{ is maximal} \quad (\text{i.e.} \; \pi \in \arg\max_{\pi \in \Pi} \Prob{\pi \models \varphi})
% \end{split}
% \end{equation}
% where $\Tau_\pi$ is the set of runs induced by $\pi$ in $\X$.
% % and $\kappa_\tau$ is the first time that $\tau$ enters a recurring component $R_i$ induced by $\pi$. 
% We use the shorthand $\mathcal{C}(s, \pi(s)) = \mathbb{E}_{a \sim \pi(s)}[\mathcal{C}(s,a)]$.

% The objective function in \eqref{eqn:main_problem} is commonly known as the average cost or gain. There may be several policies $\pi,\pi' \in \tilde{\Pi}$ that have equal gain and highest probability of LTL satisfaction. Intuitively, $\pi$ may rush to a recurring component and accumulate less cost than $\pi'$, but both still end up in indentical recurring components with equal gain. It may be desirable to pick the one that additionally yields the lower transient cost. Hence, our approach will instead pick:




% % A run $\tau = (s_0, a_0, s_1, a_1, \ldots)$ is a trajectory generated by running $\pi \in \Pi$ in $\mathcal{X}$, where each $s_i = (m_i, q_i)$ is a pair in the product space. Let $\Tau_{\pi}$ be the set of such trajectories. 

% % Since $\Tau_\pi$ forms a probability space, we can quantify the probability that $\pi \in \Pi$ satisfies $\varphi$. Recall, $\varphi$ is satisfied if the automaton states $(q_0, q_1, \ldots)$ within the run $\tau$ are contained in $F \subseteq \SState^\B$ in the LDBA infinitely often. Thus, among all (finitely many) policies $\Pi$ we can first filter on $\tilde{\Pi}$, the ones that satisfy the LTL with highest probability.

% % Next, every $\pi \in \tilde{\Pi}$ induces a Markov Chain together with $\mathcal{X}$ so we can partition $\SState = T \cup R_1 \cup \ldots \cup R_k$ where $T$ is a set of transient states (which are visited finitely often) and $R_i$ are sets of recurrent states (from which runs cannot leave and visit all states infinitely often) \cite{}. Since runs will end up in one of the $R_i$ forever, there will be an average recurring cost of traversing $R_i$. Hence, it is reasonable to look at the average cost of this policy as a criterion for policy discrimination. Ideally, we select a policy within 
% % \begin{equation*}\label{eq:opt_1}
% % \begin{split}
% % \Pi' = \arg\min_{\pi \in \tilde{\Pi}  \subseteq \Pi} \; g_\pi \left( \equiv  \mathbb{E}_{\tau \sim \Tau_{\pi}}\left[\lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^T \Cost(s_t, \pi(s_t)) \right] \right)\\
% % \end{split}
% % \end{equation*}

% % Two policies $\pi, \pi' \in \Pi'$ both have the same probability of LTL satisfaction and average cost, but they differ in their transient cost. Hence, to be slightly more selective, we aim to find
% \begin{equation*}
\begin{align*}
\tag{OPT}\label{eqn:main_problem}
\pi^\ast_{\lambda} \equiv \arg\min_{\pi \in \Pi_{\max}} \; &J_\pi + \lambda g_\pi \quad(\equiv V^P_{\pi, \lambda}) &(\text{cost optimal}) \\
\text{ where }\quad &\Pi_{\max} = \left\{\pi\in\Pi \bigg|\ \Prob{\pi \models \varphi} =\max_{\pi' \in \Pi} \Prob{\pi' \models \varphi}\right\} &(\text{prob optimal}) 
\end{align*}
We define $V^P_{\pi, \lambda} \equiv J^P_\pi + \lambda g^P_\pi$. Here, $\lambda$ represents the tradeoff between gain-optimality and transient optimality. We will often omit the dependence on $P$ and $\lambda$, when unambiguous.  

\begin{prob}[Planning with Generative Model/Simulator]
Suppose access to a generative model of the true dynamics $P^\M$ from which we can sample transitions $s' \sim P^\M(s,a)$ for any state-action pair $(s,a) \in \SState \times \A$. With probability $1-\delta$, for some error $\epsilon >0$, find a policy $\pi \in \Pi$ that simultaneously has the following properties:
\begin{equation}
(i) \;\; \Prob{\pi \models \varphi} = \Prob{\pi^\ast \models \varphi} \quad (ii)\;\; |V^{P^\M}_{\pi, \lambda} - V^{P^\M}_{\pi^\ast, \lambda}| < \epsilon 
\end{equation}
\end{prob}

% \begin{align*}
% \tag{OPT}\label{eqn:main_problem}
% \pi^\ast = \arg\min_{\pi \in \Pi} \; &V_\pi   &(\text{cost optimal}) \\
% \text{ s.t. }\quad &\pi \in \arg\max_{\pi \in \Pi} \Prob{\pi \models \varphi} &(\text{prob optimal}) 
% \end{align*}
% \end{equation*}


% An astute reader may make the claim that discounting is cleaner and for sufficiently high discount, the discount-optimal policy and the average-cost-optimal policy coincide. While this is true, there is no verifiable way to know if the chosen discount is high enough. As such, we prefer to take an approach with a verifiable formulation. We further believe that our main objective is more easily interpretable than discounted cost.

% We assume we have access to a simulator $\tilde{\X}$ of $\X$ with which we can sample $s' \sim P^{\tilde{X}}(s, a)$ for each state-action pair $(s,a)$. We assume $P^{\tilde{X}} = P^{\X}$, henceforth denoted $P$.





% \hfill
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ Accepting End Components ($\texttt{AEC}$)} 
% 	\label{algo:AEC}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE Simulator $\tilde{\X}$
%     % \STATE Call $\texttt{Sampler}(\phi_{\texttt{AEC}}(\beta), \SState)$
%     \STATE Sample $\phi_{\texttt{AEC}}(\beta)$ times in $\SState \times \A$
%     \STATE $EC = ((A_1, \A_{A_1}), \ldots, (A_m, \A_{A_m})) 
%     % \leftarrow \texttt{AEC}(\X) 
%     \leftarrow \texttt{Algorithm47}((\SState, \A, \widehat{P}))$
%     \STATE Remove $(A_i, \A_{A_i})$ from EC if $A_i \cap \SState^\ast = \varnothing$, not accepting
%     \RETURN $((A_1, \A_{A_1}), \ldots, (A_k, \A_{A_k}))$, AEC
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \hfill
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ $\texttt{Sampler}$ } 
% 	\label{algo:sampler}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE $K \in \mathbb{N}$, a set of states $S$, global $N$ transition tracker
% 	    \FOR{$s \in \SState$}
%             % \STATE $s \leftarrow S.pop()$
%             \FOR{k = 1,\ldots, K}
%                 \STATE Sample $s' \sim P(s,a)$ 
%                 \STATE Track $N(s,a,s') \pp 1, N(s,a) \pp 1$
               
%                 % \STATE If $s'$ is an unseen state, then add $s'$ to $S$ 
%             \ENDFOR
%         \ENDFOR
%     \STATE Set $\hat{P}(s,a,s') = N(s,a,s')/N(s,a)$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}

% \hfill
% \begin{minipage}{.77\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{Value Iteration $(\texttt{VI})$} 
% 	\label{algo:VI}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE Optimistic Bellman Operator $\Bellman$, Error Measure $d$, accuracy $\epsilon > 0$, $S$ states, $S_T$ terminal states, $V_T$ terminal values
% 	    \STATE Set $n=0, v_0 = 0_S, v_1 = \Bellman v_0$
% 	    \REPEAT
% 	        \STATE $n \pp 1$
% 	        \IF{$S_T$ is empty}
% 	            \STATE Shift $v_n \leftarrow v_n - v_n(0)e $ $\COMMENT{\text{Relative Value Iteration}}$
% 	        \ELSE
% 	            \STATE $v_n(s) \leftarrow V_T(s)$ for $s \in S_T$ $\COMMENT{\text{SSP}}$
% 	        \ENDIF
% 	        \STATE Apply operator $v_{n+1}, \tilde{P} \leftarrow \Bellman v_n $ $\COMMENT{\text{Bellman Backup}}$
% 	    \UNTIL{$d(v_{n+1}, v_n) > \epsilon$}
% 	\RETURN $v_{n+1}, v_n, \tilde{P}$
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \begin{minipage}{.48\textwidth}
% \begin{algorithm}[H]
% 	\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{ $\texttt{Filter}$} 
% 	\label{algo:sampler}
% 	\begin{algorithmic}[1]
% 	   \REQUIRE Gains $E=((A_1, g_1),\ldots,(A_k, g_k))$
% 	   %\STATE Set $V_T(s) = 1$ for $s \in \cup_{i=1}^k A_i$
% 	   %\STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, \cup_{i=1}^k A_i, 1)$
% 	   %\STATE Remove $(A_i, g_i)$ from $E$ if $v'(i) \neq \max(v')$
% 	    \STATE $p = 0$, the max probability of reaching
% 	    \STATE Set $G$ as the set of unique $g_i$
% 	    \WHILE{$G$ is not empty}
% 	    \STATE $g \leftarrow min(G)$, $G \leftarrow G\setminus\{g\}$
% 	    \STATE Set $A_g = \cup\{A_k \in E |g_k = g\}$
% 	    \STATE Set $V_T(s) = 1$ for $s \in A_g$
% 	   % \STATE Sample $\texttt{Sampler}(\psi(\rho), \SState \setminus \cup_{i=1}^k A_i)$
% 	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, A_g, V_T)$
% 	   % \STATE Remove $(A_i, g_i)$ from $E$ if $g_i > g$ and $v'(s) = 1$ for $s \in A_i$ arbitrary.
% 	   % \STATE Set $V = v'(s_0)$ for $s \in A_g$ arbitrary
% 	    \IF{$v'(s_0) > p$}
% 	        \STATE Set $p \leftarrow v'(s_0)$
% 	        \STATE Remove $(A_i, g_i)$ from $E$ if $g_i < g$
% 	    \ENDIF
% 	    \ENDWHILE
	    
% 	    \STATE Set $G$ as the set of unique $g_i$
% 	    \WHILE{$G$ is not empty}
% 	    \STATE $g \leftarrow min(G)$, $G \leftarrow G\setminus\{g\}$
% 	    \STATE Set $A_g = \cup\{A_k \in E |g_k = g\}$
% 	    \STATE Set $V_T(s) = 1$ for $s \in A_g$
% 	   % \STATE Sample $\texttt{Sampler}(\psi(\rho), \SState \setminus \cup_{i=1}^k A_i)$
% 	    \STATE $v', v, \tilde{P}  \leftarrow \texttt{VI}(\Bellman_{\texttt{F}}, d_{\texttt{F}}, \epsilon, \SState, A_g, V_T)$
% 	    \STATE Remove $(A_i, g_i)$ from $E$ if $g_i > g$ and $v'(s) = 1$ for $s \in A_i$ arbitrary.
% 	    \STATE Set $V = v'(s)$ for $s \in A_g$ arbitrary
% 	    \IF{$V > p$}
% 	        \STATE Set $p \leftarrow V$
% 	        \STATE Remove $(A_i, g_i)$ from $E$ if $g_i < g$
% 	    \ENDIF
% 	    \ENDWHILE
% 	\RETURN E
% 	\end{algorithmic}
% 	\end{small}
% \end{algorithm}
% \end{minipage}
% \hfill

